AspeRa: Aspect-based Rating Prediction Model

We propose a novel end-to-end Aspect-based Rating Prediction model (AspeRa) that estimates user rating based on review texts for the items and at the same time discovers coherent aspects of reviews that can be used to explain predictions or profile users. The AspeRa model uses max-margin losses for joint item and user embedding learning and a dual-headed architecture; it significantly outperforms recently proposed state-of-the-art models such as DeepCoNN, HFT, NARRE, and TransRev on two real world data sets of user reviews. With qualitative examination of the aspects and quantitative evaluation of rating prediction models based on these aspects, we show how aspect embeddings can be used in a recommender system.

==> abae.tex <==
\subsection{Neural Attention-based Aspect Extraction Model}\label{ssec:abae}

After reviewing recent approaches in learning interpretable representations for users and texts, we have decided to focus on the advanced unsupervised deep learning model called ABAE~\cite{abae}. 

As in topic modeling or the classical clustering problem setting, with ABAE we can set a finite number of topics/clusters/aspects and the goal is to determine for every document to which extent it satisfies either of topics/aspects.

From a bird's eye view, this model is an autoencoder. The main feature of ABAE is the reconstruction loss between bag of word embeddings used as the sentence representation and a linear combination of aspect embeddings. A sentence embedding is not an actual bag of words, it is weighted by the so called \emph{self-attention}, an attention mechanism where the values are word embeddings and the key is the mean embedding of words in a sentence.

The first step in ABAE is to compute the embedding $z_s \in \mathbb{R}^d$ for a sentence $s$:
  \begin{align*}
    z_s &= \sum_{i=1}^n a_i e_{w_i},
  \end{align*}
where $e_{w_i}$ is a word embedding for a word $w_i$, $e \in \mathbb{R}^d$. As word vectors the authors use \emph{word2vec} embeddings trained with the skip-gram model \cite{mikolov2013distributed}.

Attention weights $a_i$ are computed as a multiplicative self-attention model:
  \begin{align*}
    a_i &= \textrm{softmax}(e_{w_i}^{\textrm{T}} \cdot A \cdot y_s), \\
    y_s &= \sum_{i=1}^n e_{w_i},
  \end{align*}
where $y_s$ is the simple mean of word embeddings in a sentence, and $A \in \mathbb{R}^{d \times d}$ is the learned attention model.

The second step is to compute the aspect-based sentence representation $r_s \in \mathbb{R}^d$ from an aspect embeddings matrix $T \in \mathbb{R}^{k \times d}$, where $k$ is the number of aspects:
  \begin{align*}
    p_s &= \textrm{softmax}(W \cdot z_s + b), \\
    r_s &= T^{\textrm{T}} \cdot p_s,
  \end{align*}
where $p_s \in \mathbb{R}^k$ is the vector of probability weights over $k$ aspect embeddings, and $W \in \mathbb{R}^{k \times d}$, $b\in\mathbb{R}^k$ are the parameters of a multi-class logistic regression model.

To train the model, ABAE uses reconstruction error as the cosine distance between $r_s$ and $z_s$ with a contrastive max-margin objective function~\cite{weston2011wsabie}. In addition, an orthogonality penalty term is added to the objective, which tries to make the aspect embedding matrix $T$ to produce as diverse aspect embeddings as possible. %The entire architecture is presented on Fig.~\ref{fig:fig5}.

%For the implementation of the ABAE model for our purposes, all reviews from the corpora mentioned above (see Section~\ref{sec:data}) have been split into individual sentences and normalized (lemmatized etc.).

%The ABAE model appears to be a suitable solution for the extraction of product features, advantages, and flaws that users discuss, e.g. on Amazon. However, qualitative as well as quantitative analysis has shown that quite a few challenges still remain for our case, where we would like to use these aspects for further user profiling and recommendations. In the next section, we pose the main questions and answer them with our novel contributions.
\begin{comment}
\begin{figure}[t]
    \centering
\includegraphics[width=12cm,keepaspectratio]{pic/ABAE.png}
    \caption{The ABAE architecture.}
    \label{fig:fig5}
\end{figure}
\end{comment}

